A Novel Simulation-Based Quality Metric for Evaluating Grasps on 3D Deformable Objects

Evaluation of grasps on deformable 3D objects is a little-studied problem, even if the applicability of rigid object grasp quality measures for deformable ones is an open question. A central issue with most quality measures is their dependence on contact points which for deformable objects depend on the deformations. This paper proposes a grasp quality measure for deformable objects that uses information about object deformation to calculate the grasp quality. Grasps are evaluated by simulating the deformations during grasping and predicting the contacts between the gripper and the grasped object. The contact information is then used as input for a new grasp quality metric to quantify the grasp quality. The approach is benchmarked against two classical rigid-body quality metrics on over 600 grasps in the Isaac gym simulation and over 50 real-world grasps. Experimental results show an average improvement of 18\% in the grasp success rate for deformable objects compared to the classical rigid-body quality metrics.

==> sections/method.tex <==
% \newpage
% \clearpage
\section{Gravity-resistant quality metric for 3D deformable objects}
\label{sec:metrics}
\begin{figure}
    \centering
    \def\svgwidth{\linewidth}
     {\color{black} \fontsize{15}{15}%\selectfont\sf
    \input{figures_tex/intersect.pdf_tex}}       
    \caption{The $\mathcal{P}(t)$ (blue polygon) and $\mathcal{P}_{gravity}$ (red sphere) are projected into force space. The proposed quality metric is then determined as the distance from the wrench space origin to its closest intersection point (green dot) of the two wrench spaces.}
    \label{fig:intersect}
    \vspace{-0.5cm}
\end{figure}
We propose to derive a quality metric for deformable objects based on the mechanical wrench space analysis. As discussed in the previous section, we evaluate a grasp by quantifying how well it can keep the target object under gravity. Our quality metric is inspired from \cite{inspire14}. However, that work only considers the stability of soft-finger grasp on rigid objects under gravity and not the stability of rigid grasps on non-rigid objects.




%We propose a quality metric derived from mechanical wrench space analysis that is applicable for deformable objects. As discussed in \secref{sec:prob}, we evaluate a grasp by quantifying how well a grasp can keep the target object under gravity. In addition, to apply the quality metric to different manipulation tasks rather than just lifting, we consider the situation where the direction of the gravity is unknown. Our quality metric is inspired by the one proposed in \cite{inspire14} in which evaluates the stability of soft-finger grasp under gravity but with some important modifications to tailor it to our application on deformable objects.

% First, let us define the wrench of a grasp 
    
Let us recall $\mathcal{P}(t)$ is the 6D \gls{gws} of a grasp configuration at a certain time-step. It is noteworthy that we consider the origin of the \gls{gws} at the contact centroid instead of having it at the object center-of-mass. The reason for this modification is that we want to have a closer look at the behavior of the interaction between the gripper and the target object at the contact regions. Here, let $\mathcal{P}_{gravity}$ be the 6D wrench space of the gravity acting on the object. As we want to evaluate a grasp in the case where the gravitational force direction is unknown, $\mathcal{P}_{gravity}$ consists of the wrench of gravitational forces in 16 directions regularly spaced in a unit sphere (as visualized in \figref{fig:title}). Afterward, we compute the intersection of the two wrench spaces as
\begin{equation*}
    \mathcal{P}_{int}(t) = \mathcal{P}(t) \cap \mathcal{P}_{gravity} 
\end{equation*}
Which leads us to define our new quality metric as the distance from the origin of the wrench space to the closest intersection point
\begin{equation*}
    \mathcal{Q}(t) = \min_{w_i \in \mathcal{P}_{int}(t)} || w_i || 
\end{equation*}


For visualization purposes, we show the components and the proposed quality metric in a 3D plot in \figref{fig:intersect}. This metric indicates which direction the target can be displaced the most by the gravitational force and how much a grasp can be maintained against that gravitational force. By continuously determining the \gls{gws} $\mathcal{P}(t)$, the quality metric is repeatedly calculated to evaluate the grasp candidate during the grasp. By doing this we are able to take into account the effect of object deformation in quantifying the goodness of a grasp configuration.


==> sections/problem_formulation.tex <==
% \clearpage
% \newpage
\section{Problem Formulation}
\label{sec:prob}
In this work we address the problem of evaluating parallel-jaw grasps on 3D deformable objects lying on a supporting surface. This implies producing a quality-metric $q$ that measures how well a grasp can keep the object restrained even if affected by disturbing forces or torques. Based on previous work \cite{defgraspsim,lin_feel3d,com16}, the main disturbance that causes grasp failure is gravity. Therefore, we propose a quality metric that can quantify how well a grasp can safely keep the object under the effect of gravity.

We assume the geometry and stiffness of the target object are known and that the object's origin is at its center-of-mass. We also consider that the direction of gravity is unknown.

As deformable objects deform under interaction forces, the contact locations also depend on the forces exerted on the object. The contact locations during the grasp are thus different from the initial locations. There should be multiple contact points between the gripper and the object rather than two during the interaction due to the object deformation. Therefore, it is crucial to track the contact locations during the grasp and measure its quality on the fly. We target this problem by considering a grasp with multiple contacts and we propose using \gls{fem} to track and obtain the information of contact points such as contact locations, normal directions, etc. More formally, let us consider a grasp with $N$ contacts, we denote $\bm{w}_i \in \mathbb{R}^6$ as the contact wrench that consists of force $\bm{f}_i$ and torque $\bm{\mathcal{T}}_i$ applied at the \textit{i}-th contact. Using the frictional contact point model, the contact wrench at location $x_i$ is expressed as:
\begin{equation*}
     \bm{w}_i = \left[\begin{array}{c}\bm{f}_i\\\bm{\mathcal{T}}_i\end{array}\right] = \left[\begin{array}{c}\bm{f}_i\\x_i \times \bm{f}_i\end{array}\right],
\end{equation*}
We then repeatedly determine \gls{gws} $\mathcal{P}$ to understand the behavior of the grasp during the grasping procedure. $\mathcal{P}(t)$ is defined as the convex hull of the contact wrenches at a certain time step and it is expressed as:
\begin{equation*}
     \mathcal{P}(t) = ConvexHull\left(\bigcup_{i=1}^{n}w_i\right),
\end{equation*}
$\mathcal{P}(t)$  will then be used to evaluate the quality of the grasp.

To quantify the quality of a grasp, we aim to formulate a \gls{gqm}. We consider a grasp to be successful if only it completes a manipulation task without dropping the target object. As pointed out in the literature \cite{defgraspsim,lin_feel3d,com16}, the major disturbance that causes grasp failure is gravity. During the manipulation, the deformable objects usually exhibit gravity-induced deformation and this deformation may bring instability to the grasp. Therefore, we propose a quality metric that can quantify how well a grasp can safely keep the object under the effect of gravity. 


